Measurement of $WW/WZ \to \ell \nu q q^{\prime}$ production with the hadronically decaying boson reconstructed as one or two jets in $pp$ collisions at $\sqrt{s}=8$ TeV with ATLAS, and constraints on anomalous gauge couplings

This paper presents a study of the production of $WW$ or $WZ$ boson pairs, with one $W$ boson decaying to $e\nu$ or $\mu\nu$ and one $W$ or $Z$ boson decaying hadronically. The analysis uses 20.2 fb$^{-1}$ of $\sqrt{s}=8$ TeV $pp$ collision data, collected by the ATLAS detector at the Large Hadron Collider. Cross-sections for $WW/WZ$ production are measured in high-$p_{T}$ fiducial regions defined close to the experimental event selection. The cross-section is measured for the case where the hadronically decaying boson is reconstructed as two resolved jets, and the case where it is reconstructed as a single jet. The transverse momentum distribution of the hadronically decaying boson is used to search for new physics. Observations are consistent with the Standard Model predictions, and $95\%$ confidence intervals are calculated for parameters describing anomalous triple gauge-boson couplings.

==> Auxiliary.tex <==



\begin{figure}[htbp]
\begin{center}
\subfigure[]{
 \includegraphics[width=0.47\textwidth,keepaspectratio]{templates_resolved_mjj_signal.pdf}
}
\subfigure[]{
 \includegraphics[width=0.47\textwidth,keepaspectratio]{WWvsWZboosted.pdf}  
}
\caption{
(a) Comparison of the $\mjjless$ distributions for the $WW$ and $WZ$ processes, in the
\resolved\ channel.
(b) Comparison of the $\mJ$ distributions for the $WW$ and $WZ$ processes, in the
\boosted\ channel.
}
\label{auxfig:templates_signalWWWZ}
\end{center}
\end{figure}


 


\begin{figure}[htbp]
\begin{center}
\subfigure[]{
 \includegraphics[width=0.47\textwidth,keepaspectratio]{prefit/met.pdf}
}
\subfigure[]{
 \includegraphics[width=0.47\textwidth,keepaspectratio]{prefit/ptlep.pdf}
}
\subfigure[]{
 \includegraphics[width=0.47\textwidth,keepaspectratio]{prefit/ptW.pdf}
}
\subfigure[]{
 \includegraphics[width=0.47\textwidth,keepaspectratio]{prefit/mt.pdf}
}
\caption{
Data-MC comparisons in the \resolved\ channel, prior to performing the cross-section fit.
The distributions shown are
(a) $\met$,
(b) $p_T(\ell)$. 
(c) $\pT(\Wlep)$, and
(d) $\MT$, 
The hatched bands indicate the systematic uncertainty on the prediction. Overflow is included in the last bin.
}
\label{auxfig:prefit_dataMC_resolved_1}
\end{center}
\end{figure}



\begin{figure}[htbp]
\begin{center}

\subfigure[]{
 \includegraphics[width=0.47\textwidth,keepaspectratio]{prefit/ptj1.pdf}
}
\subfigure[]{
 \includegraphics[width=0.47\textwidth,keepaspectratio]{prefit/dR.pdf}
}
\caption{
Data-MC comparisons in the \resolved\ channel, prior to performing the cross-section fit.
The distributions shown are
(a) $\pT$ of the leading jet and
(b) $\Delta R$ between the leading jet and sub-leading jet. 
The hatched bands indicate the systematic uncertainty on the prediction. Overflow is included in the last bin.
}
\label{auxfig:prefit_dataMC_resolved_2}
\end{center}
\end{figure}
  

\begin{figure}[htbp]   
\begin{center}
\subfigure[]{
 \includegraphics[width=0.47\textwidth,keepaspectratio]{prefit_boosted/kin_MET.pdf}
}
\subfigure[]{
 \includegraphics[width=0.47\textwidth,keepaspectratio]{prefit_boosted/akt10_leptonPt.pdf}
}
\subfigure[]{
 \includegraphics[width=0.47\textwidth,keepaspectratio]{prefit_boosted/ptWlv.pdf}
}
\subfigure[]{
 \includegraphics[width=0.47\textwidth,keepaspectratio]{prefit_boosted/akt10_mT.pdf}
}
\caption{
Data-MC comparisons in the \boosted\ channel, prior to performing the cross-section fit.  The
distributions shown are
(a) $\met$, 
(b) $\pT(\ell)$,
(c) $\pT(\Wlep)$,    
and 
(d) $\MT$.
The hatched bands indicate the systematic uncertainty on the prediction. Overflow is included in the last bin.
}
\label{auxfig:prefit_dataMC_boosted_1}
\end{center}
\end{figure}


\begin{figure}[htbp]   
\begin{center}
 \includegraphics[width=0.47\textwidth,keepaspectratio]{prefit_boosted/akt10_nrealVetoJets.pdf}
\caption{
Number of veto jets in the \boosted\ channel before applying the jet veto. Only the 0-jet bin is selected. 
The hatched band indicates the systematic uncertainty on the prediction. Overflow is included in the last bin.
}
\label{auxfig:vetoJetMult}
\end{center}
\end{figure}





\begin{figure}[htbp]
\begin{center}
 \includegraphics[width=0.47\textwidth,keepaspectratio]{aTGC_pTjj_resolved_sideband.pdf}
\caption{
 The observed $\pTjj$ distribution in the \resolved\ 
aTGC sideband control region.
The expected BSM enhancements due to anomalous values of the EFT parameter $\cwww$ 
are also shown, for $\cwww=4~\tevminSq$ and $\cwww=8~\tevminSq$. 
The hatched bands indicate the systematic uncertainty on the SM prediction.
The histograms are displayed with the binning that is used for the computation
of the confidence intervals for the aTGC and EFT parameters.
The last bin includes overflow.
}
\label{fig:aTGCfitDistObservedSideband}
\end{center}
\end{figure}


\FloatBarrier


\begin{table}[htbp]
\begin{center}
{ \footnotesize
\begin{tabular}{c|cccccc|cccc} 
\hline \hline
  & \multicolumn{10}{c}{\resolved\ channel} \\
 &  \multicolumn{6}{c}{SR } &  \multicolumn{4}{c}{sideband CR} \\
\hline
bin & 1 & 2 & 3 & 4 & 5 & 6 &  1 & 2 & 3 & 4  \\
\hline
 $\Vjet$ &  30472.33 &  3718.25 &  614.53 &  133.55 &  8.11 &  0.60 &  89033.62 &  12297.41 &  2218.02 &  10.71 \\
 Top-quark &  4689.92 &  663.11 &  71.02 &  4.23 &  0.26 &  0.00 &  9879.75 &  1120.07 &  173.27 &  0.84 \\
 Multijet &  813.64 &  94.39 &  25.41 &  0.81 &  0.00 &  0.00 &  2352.87 &  346.36 &  55.75 &  0.00 \\ 
$WV$ (SM) &  1814.33 &  348.74 &  67.27 &  11.10 &  0.45 &  0.33 &  1061.49 &  172.55 &  55.22 &  0.21 \\
\hline
$WV$ ($\cwww=8~\tevminSq$)   &   38.16 &  88.19 &  73.91 &  38.60 &  5.67 &  1.02 &  30.03 &  27.49 &  36.86 &  3.80 \\
$WV$ ($\cwww=4~\tevminSq$)   &   2.22 &  20.58 &  18.35 &  9.71 &  1.43 &  0.26 &  7.84 &  7.47 &  9.70 &  0.96 \\
\hline
Data &  37569 &  4781 &  712 &  146 &  10 &  0 &  104538 &  14196 &  2538 &  12 \\
\hline\hline
\end{tabular}
}
\caption{The expected number of events passing the final event
selection in the \resolved\ channel,  in each $\pTjj$ bin. The expected number of background and signal events are given,
together with the number of events observed in data. The numbers correspond to Figures~\ref{fig:aTGCfitDistObservedBoosted}
 and \ref{fig:aTGCfitDistObservedSideband}.
The BSM numbers do not include the SM $WV$ contribution, so the SM and BSM $WV$ numbers should be added together.
The numbers correspond to the raw event yields, not divided by the bin widths.
The six bins in the SR have the following bin boundaries: $(100, 200, 300, 400, 600, 800, \infty)~\gev$.
The four bins in the sideband CR have the following bin boundaries: $(100, 200, 300, 700, \infty)~\gev$.
}
\label{tab:BinByBinYieldsResolved}
\end{center}
\end{table}




\begin{table}[htbp]
\begin{center}
{ \footnotesize
\begin{tabular}{c|cccccc} 
\hline \hline
  & \multicolumn{6}{c}{\boosted\ channel} \\
\hline
bin & 1 & 2 & 3 & 4 & 5 & 6  \\
\hline
 $\Vjet$ &  3417.76 &  653.07 &  147.77 &  41.86 &  13.34 &  9.00 \\
 Top-quark & 517.80 &  67.70 &  9.36 &  1.54 &  1.08 &  0.23 \\
 Multijet & 107.35 &  19.40 &  0.55 &  1.74 &  1.43 &  0.00 \\
$WV$ (SM) &  363.85 &  83.61 &  22.89 &  7.58 &  2.12 &  1.30 \\
\hline
$WV$ ($\cwww=8~\tevminSq$)   &   112.94 &  104.77 &  79.72 &  55.64 &  36.70 &  61.32 \\
$WV$ ($\cwww=4~\tevminSq$)   &   26.70 &  26.07 &  20.03 &  13.99 &  9.22 &  15.38 \\
\hline
Data &  4407 &  749 &  191 &  42 &  13 &  8 \\
\hline\hline
\end{tabular}
}
\caption{The expected number of events passing the final event
selection in the \boosted\ channel,  in each $\pTJ$ bin. The expected number of background and signal events are given,
together with the number of events observed in data. The numbers correspond to Figure~\ref{fig:aTGCfitDistObservedBoosted}.
The numbers correspond to the raw event yields, not divided by the bin widths.
The BSM numbers do not include the SM $WV$ contribution, so the SM and BSM $WV$ numbers should be added together.
The six bins have the following bin boundaries: $(100, 200, 300, 400, 500, 600, 700, \infty)~\gev$.
}
\label{tab:BinByBinYieldsBoosted}
\end{center}
\end{table}

